Optimizing Quantum Embedding using Genetic Algorithm for QML Applications

Quantum Embeddings (QE) are essential for loading classical data into quantum systems for Quantum Machine Learning (QML). The performance of QML algorithms depends on the type of QE and how features are mapped to qubits. Traditionally, the optimal embedding is found through optimization, but we propose framing it as a search problem instead. In this work, we use a Genetic Algorithm (GA) to search for the best feature-to-qubit mapping. Experiments on the MNIST and Tiny ImageNet datasets show that GA outperforms random feature-to-qubit mappings, achieving 0.33-3.33 (MNIST) and 0.5-3.36 (Tiny ImageNet) higher fitness scores, with up to 15% (MNIST) and 8.8% (Tiny ImageNet) reduced runtime. The GA approach is scalable with both dataset size and qubit count. Compared to existing methods like Quantum Embedding Kernel (QEK), QAOA-based embedding, and QRAC, GA shows improvements of 1.003X, 1.03X, and 1.06X, respectively.

==> 5_Results.tex <==
\section{Results}

% \begin{table*}[t]
% \centering
% \caption{MNIST low qubit count results. Note that rs $=$ random selection, Q $=\#$qubits .}
% \label{tab:mnist_low_qubit_count}
% \makebox[\textwidth][c]{
% \begin{tabular}{|l|llll|llll|}
% \hline
%                        & \multicolumn{4}{l|}{\textbf{Noiseless fitness scores}}                                                                                                                                                                & \multicolumn{4}{l|}{\textbf{Noisy fitness scores}}                                                                                                                                                                    \\ \hline
% \textbf{(c$_1$,c$_2$,} \\ \textbf{Q)} & \multicolumn{1}{l|}{\textbf{mean(rs)}} & \multicolumn{1}{l|}{\textbf{best(rs)}} & \multicolumn{1}{l|}{\textbf{GA\_best}} & \textbf{GA\_best\_config}                                     & \multicolumn{1}{l|}{\textbf{mean(rs)}} & \multicolumn{1}{l|}{\textbf{best(rs)}} & \multicolumn{1}{l|}{\textbf{GA\_best}} & \textbf{GA\_best\_config}                                     \\ \hline
% \textit{(4,9,3)}       & \multicolumn{1}{l|}{70.04}                    & \multicolumn{1}{l|}{73.43}                    & \multicolumn{1}{l|}{72.12}             & ($f_4$,$f_0$,$f_1$,$f_5$,$f_2$,$f_3$)                         & \multicolumn{1}{l|}{64.25}                    & \multicolumn{1}{l|}{67.15}                    & \multicolumn{1}{l|}{65.50}             & ($f_3$,$f_0$,$f_2$,$f_1$,$f_4$,$f_5$)                         \\ \hline
% \textit{(3,8,3)}       & \multicolumn{1}{l|}{79.30}                    & \multicolumn{1}{l|}{82.06}                    & \multicolumn{1}{l|}{82.37}             & ($f_1$,$f_5$,$f_0$,$f_2$,$f_3$,$f_4$)                         & \multicolumn{1}{l|}{70.44}                    & \multicolumn{1}{l|}{72.78}                    & \multicolumn{1}{l|}{70.88}             & ($f_2$,$f_5$,$f_3$,$f_4$,$f_0$,$f_1$)                         \\ \hline
% \textit{(2,6,3)}       & \multicolumn{1}{l|}{87.49}                    & \multicolumn{1}{l|}{91.93}                    & \multicolumn{1}{l|}{91.18}             & ($f_3$,$f_2$,$f_1$,$f_4$,$f_4$,$f_0$)                         & \multicolumn{1}{l|}{77.59}                    & \multicolumn{1}{l|}{81.70}                    & \multicolumn{1}{l|}{78.60}             & ($f_5$,$f_3$,$f_0$,$f_2$,$f_1$,$f_4$)                         \\ \hline
% \textit{(0,3,3)}       & \multicolumn{1}{l|}{90.88}                    & \multicolumn{1}{l|}{95.5}                     & \multicolumn{1}{l|}{93.68}             & ($f_4$,$f_3$,$f_5$,$f_2$,$f_1$,$f_0$)                         & \multicolumn{1}{l|}{79.94}                    & \multicolumn{1}{l|}{83.60}                    & \multicolumn{1}{l|}{80.46}             & ($f_3$,$f_0$,$f_4$,$f_5$,$f_1$,$f_2$)                         \\ \hline
% \textit{(1,4,3)}       & \multicolumn{1}{l|}{96.90}                    & \multicolumn{1}{l|}{98.31}                    & \multicolumn{1}{l|}{98.25}             & ($f_3$,$f_2$,$f_1$,$f_4$,$f_0$,$f_5$)                         & \multicolumn{1}{l|}{84.43}                    & \multicolumn{1}{l|}{88.62}                    & \multicolumn{1}{l|}{86.79}             & ($f_1$,$f_0$,$f_2$,$f_5$,$f_3$,$f_4$)                         \\ \hline
% \textit{(0,1,3)}       & \multicolumn{1}{l|}{95.64}                    & \multicolumn{1}{l|}{98.62}                    & \multicolumn{1}{l|}{98.68}             & ($f_3$,$f_5$,$f_4$,$f_2$,$f_0$,$f_1$)                         & \multicolumn{1}{l|}{32.12}                    & \multicolumn{1}{l|}{88.56}                    & \multicolumn{1}{l|}{86.28}             & ($f_1$,$f_3$,$f_4$,$f_5$,$f_0$,$f_2$)                         \\ \hline
% \textit{(4,9,4)}       & \multicolumn{1}{l|}{73.81}                    & \multicolumn{1}{l|}{80.62}                    & \multicolumn{1}{l|}{79.06}             & ($f_7$,$f_2$,$f_6$,$f_0$,$f_4$,$f_5$,$f_3$,$f_1$)             & \multicolumn{1}{l|}{66.36}                    & \multicolumn{1}{l|}{69.03}                    & \multicolumn{1}{l|}{71.63}             & ($f_0$,$f_6$,$f_3$,$f_7$,$f_4$,$f_5$,$f_2$,$f_1$)             \\ \hline
% \textit{(3,8,4)}       & \multicolumn{1}{l|}{83.74}                    & \multicolumn{1}{l|}{87.25}                    & \multicolumn{1}{l|}{87.5}              & ($f_7$,$f_2$,$f_6$,$f_0$,$f_4$,$f_5$,$f_3$,$f_1$)             & \multicolumn{1}{l|}{73.73}                    & \multicolumn{1}{l|}{76.70}                    & \multicolumn{1}{l|}{78.12}             & ($f_4$,$f_2$,$f_1$,$f_3$,$f_5$,$f_6$,$f_0$,$f_7$)             \\ \hline
% \textit{(2,6,4)}       & \multicolumn{1}{l|}{87.07}                    & \multicolumn{1}{l|}{91.31}                    & \multicolumn{1}{l|}{89.68}             & ($f_7$,$f_1$,$f_6$,$f_4$,$f_5$,$f_2$,$f_3$,$f_0$)             & \multicolumn{1}{l|}{76.42}                    & \multicolumn{1}{l|}{80.50}                    & \multicolumn{1}{l|}{82.13}             & ($f_6$,$f_1$,$f_2$,$f_3$,$f_4$,$f_0$,$f_5$,$f_7$)             \\ \hline
% \textit{(0,3,4)}       & \multicolumn{1}{l|}{90.21}                    & \multicolumn{1}{l|}{95.56}                    & \multicolumn{1}{l|}{93.06}             & ($f_3$,$f_4$,$f_6$,$f_7$,$f_0$,$f_1$,$f_2$,$f_5$)             & \multicolumn{1}{l|}{77.86}                    & \multicolumn{1}{l|}{81.59}                    & \multicolumn{1}{l|}{83.93}             & ($f_5$,$f_0$,$f_7$,$f_2$,$f_4$,$f_3$,$f_1$,$f_6$)             \\ \hline
% \textit{(1,4,4)}       & \multicolumn{1}{l|}{97.04}                    & \multicolumn{1}{l|}{98.75}                    & \multicolumn{1}{l|}{98.62}             & ($f_3$,$f_0$,$f_2$,$f_5$,$f_1$,$f_6$,$f_7$,$f_4$)             & \multicolumn{1}{l|}{82.77}                    & \multicolumn{1}{l|}{87.59}                    & \multicolumn{1}{l|}{90.08}             & ($f_3$,$f_2$,$f_5$,$f_4$,$f_7$,$f_6$,$f_1$,$f_0$)             \\ \hline
% \textit{(0,1,4)}       & \multicolumn{1}{l|}{95.14}                    & \multicolumn{1}{l|}{98.56}                    & \multicolumn{1}{l|}{98.55}             & ($f_6$,$f_7$,$f_0$,$f_1$,$f_2$,$f_4$,$f_5$,$f_3$)             & \multicolumn{1}{l|}{80.94}                    & \multicolumn{1}{l|}{85.75}                    & \multicolumn{1}{l|}{90.61}             & ($f_5$,$f_2$,$f_1$,$f_4$,$f_0$,$f_3$,$f_6$,$f_7$)             \\ \hline
% \textit{(4,9,5)}       & \multicolumn{1}{l|}{74.38}                    & \multicolumn{1}{l|}{80.93}                    & \multicolumn{1}{l|}{78.87}             & ($f_0$,$f_9$,$f_5$,$f_1$,$f_7$,$f_8$,$f_2$,$f_4$,$f_3$,$f_6$) & \multicolumn{1}{l|}{65.42}                    & \multicolumn{1}{l|}{68.68}                    & \multicolumn{1}{l|}{70.35}             & ($f_2$,$f_6$,$f_9$,$f_4$,$f_1$,$f_5$,$f_8$,$f_3$,$f_0$,$f_7$) \\ \hline
% \textit{(3,8,5)}       & \multicolumn{1}{l|}{82.48}                    & \multicolumn{1}{l|}{86.87}                    & \multicolumn{1}{l|}{85.12}             & ($f_3$,$f_5$,$f_4$,$f_2$,$f_6$,$f_1$,$f_7$,$f_8$,$f_9$,$f_0$) & \multicolumn{1}{l|}{69.98}                    & \multicolumn{1}{l|}{73.6}                     & \multicolumn{1}{l|}{76.03}             & ($f_0$,$f_6$,$f_7$,$f_9$,$f_2$,$f_8$,$f_4$,$f_1$,$f_5$,$f_3$) \\ \hline
% \textit{(2,6,5)}       & \multicolumn{1}{l|}{86.68}                    & \multicolumn{1}{l|}{92.56}                    & \multicolumn{1}{l|}{90.37}             & ($f_7$,$f_2$,$f_3$,$f_5$,$f_1$,$f_9$,$f_0$,$f_8$,$f_4$,$f_6$) & \multicolumn{1}{l|}{73.31}                    & \multicolumn{1}{l|}{76.73}                    & \multicolumn{1}{l|}{79.65}             & ($f_8$,$f_7$,$f_0$,$f_2$,$f_1$,$f_6$,$f_5$,$f_9$,$f_3$,$f_4$) \\ \hline
% \textit{(0,3,5)}       & \multicolumn{1}{l|}{88.69}                    & \multicolumn{1}{l|}{95.5}                     & \multicolumn{1}{l|}{91.68}             & ($f_6$,$f_3$,$f_5$,$f_8$,$f_7$,$f_9$,$f_2$,$f_4$,$f_1$,$f_0$) & \multicolumn{1}{l|}{73.38}                    & \multicolumn{1}{l|}{78.08}                    & \multicolumn{1}{l|}{81.73}             & ($f_3$,$f_5$,$f_0$,$f_9$,$f_1$,$f_6$,$f_2$,$f_7$,$f_8$,$f_4$) \\ \hline
% \textit{(1,4,5)}       & \multicolumn{1}{l|}{95.89}                    & \multicolumn{1}{l|}{99.18}                    & \multicolumn{1}{l|}{98.37}             & ($f_6$,$f_8$,$f_2$,$f_9$,$f_5$,$f_4$,$f_3$,$f_7$,$f_1$,$f_0$) & \multicolumn{1}{l|}{79.31}                    & \multicolumn{1}{l|}{83.81}                    & \multicolumn{1}{l|}{86.25}             & ($f_3$,$f_8$,$f_2$,$f_1$,$f_6$,$f_9$,$f_0$,$f_7$,$f_5$,$f_4$) \\ \hline
% \textit{(0,1,5)}       & \multicolumn{1}{l|}{95.64}                    & \multicolumn{1}{l|}{98.68}                    & \multicolumn{1}{l|}{98.37}             & (($f_6$,$f_3$),($f_0$,$f_9$),($f_5$,$f_8$),($f_4$,$f_2$),($f_7$,$f_1$)) & \multicolumn{1}{l|}{78.75}                    & \multicolumn{1}{l|}{86.33}                    & \multicolumn{1}{l|}{87.0}              & (($f_4$,$f_1$),($f_9$,$f_5$),($f_0$,$f_2$),($f_7$,$f_3$),($f_8$,$f_6$)) \\ \hline
% \end{tabular}
% }
% \end{table*}

\begin{table*}[t]
\centering
\caption{MNIST low qubit count results. Note that rs $=$ random selection, Q $=\#$qubits .}
\label{tab:mnist_low_qubit_count}
\begin{tabular}{|l|llll|llll|}
\hline
                       & \multicolumn{4}{l|}{\textbf{Noiseless fitness scores}}                                                                                                                                 & \multicolumn{4}{l|}{\textbf{Noisy fitness scores}}                                                                                                                                     \\ \hline
\textbf{(c$_1$,c$_2$,} & \multicolumn{2}{l|}{\textbf{RS}}                                        & \multicolumn{2}{l|}{\textbf{GA}}                                                                             & \multicolumn{2}{l|}{\textbf{RS}}                                        & \multicolumn{2}{l|}{\textbf{GA}}                                                                             \\ \cline{2-9} 
\textbf{Q)}            & \multicolumn{1}{l|}{\textbf{mean}} & \multicolumn{1}{l|}{\textbf{best}} & \multicolumn{1}{l|}{\textbf{best}} & \textbf{best\_config}                                                   & \multicolumn{1}{l|}{\textbf{mean}} & \multicolumn{1}{l|}{\textbf{best}} & \multicolumn{1}{l|}{\textbf{best}} & \textbf{best\_config}                                                   \\ \hline
\textit{4,9,3}         & \multicolumn{1}{l|}{70.04}         & \multicolumn{1}{l|}{73.43}         & \multicolumn{1}{l|}{72.12}         & ($f_4$,$f_0$,$f_1$,$f_5$,$f_2$,$f_3$)                                   & \multicolumn{1}{l|}{64.25}         & \multicolumn{1}{l|}{67.15}         & \multicolumn{1}{l|}{65.50}         & ($f_3$,$f_0$,$f_2$,$f_1$,$f_4$,$f_5$)                                   \\ \hline
\textit{3,8,3}         & \multicolumn{1}{l|}{79.30}         & \multicolumn{1}{l|}{82.06}         & \multicolumn{1}{l|}{82.37}         & ($f_1$,$f_5$,$f_0$,$f_2$,$f_3$,$f_4$)                                   & \multicolumn{1}{l|}{70.44}         & \multicolumn{1}{l|}{72.78}         & \multicolumn{1}{l|}{70.88}         & ($f_2$,$f_5$,$f_3$,$f_4$,$f_0$,$f_1$)                                   \\ \hline
\textit{2,6,3}         & \multicolumn{1}{l|}{87.49}         & \multicolumn{1}{l|}{91.93}         & \multicolumn{1}{l|}{91.18}         & ($f_3$,$f_2$,$f_1$,$f_4$,$f_4$,$f_0$)                                   & \multicolumn{1}{l|}{77.59}         & \multicolumn{1}{l|}{81.70}         & \multicolumn{1}{l|}{78.60}         & ($f_5$,$f_3$,$f_0$,$f_2$,$f_1$,$f_4$)                                   \\ \hline
\textit{0,3,3}         & \multicolumn{1}{l|}{90.88}         & \multicolumn{1}{l|}{95.5}          & \multicolumn{1}{l|}{93.68}         & ($f_4$,$f_3$,$f_5$,$f_2$,$f_1$,$f_0$)                                   & \multicolumn{1}{l|}{79.94}         & \multicolumn{1}{l|}{83.60}         & \multicolumn{1}{l|}{80.46}         & ($f_3$,$f_0$,$f_4$,$f_5$,$f_1$,$f_2$)                                   \\ \hline
\textit{1,4,3}         & \multicolumn{1}{l|}{96.90}         & \multicolumn{1}{l|}{98.31}         & \multicolumn{1}{l|}{98.25}         & ($f_3$,$f_2$,$f_1$,$f_4$,$f_0$,$f_5$)                                   & \multicolumn{1}{l|}{84.43}         & \multicolumn{1}{l|}{88.62}         & \multicolumn{1}{l|}{86.79}         & ($f_1$,$f_0$,$f_2$,$f_5$,$f_3$,$f_4$)                                   \\ \hline
\textit{0,1,3}         & \multicolumn{1}{l|}{95.64}         & \multicolumn{1}{l|}{98.62}         & \multicolumn{1}{l|}{98.68}         & ($f_3$,$f_5$,$f_4$,$f_2$,$f_0$,$f_1$)                                   & \multicolumn{1}{l|}{32.12}         & \multicolumn{1}{l|}{88.56}         & \multicolumn{1}{l|}{86.28}         & ($f_1$,$f_3$,$f_4$,$f_5$,$f_0$,$f_2$)                                   \\ \hline
\textit{4,9,4}         & \multicolumn{1}{l|}{73.81}         & \multicolumn{1}{l|}{80.62}         & \multicolumn{1}{l|}{79.06}         & ($f_7$,$f_2$,$f_6$,$f_0$,$f_4$,$f_5$,$f_3$,$f_1$)                       & \multicolumn{1}{l|}{66.36}         & \multicolumn{1}{l|}{69.03}         & \multicolumn{1}{l|}{71.63}         & ($f_0$,$f_6$,$f_3$,$f_7$,$f_4$,$f_5$,$f_2$,$f_1$)                       \\ \hline
\textit{3,8,4}         & \multicolumn{1}{l|}{83.74}         & \multicolumn{1}{l|}{87.25}         & \multicolumn{1}{l|}{87.5}          & ($f_7$,$f_2$,$f_6$,$f_0$,$f_4$,$f_5$,$f_3$,$f_1$)                       & \multicolumn{1}{l|}{73.73}         & \multicolumn{1}{l|}{76.70}         & \multicolumn{1}{l|}{78.12}         & ($f_4$,$f_2$,$f_1$,$f_3$,$f_5$,$f_6$,$f_0$,$f_7$)                       \\ \hline
\textit{2,6,4}         & \multicolumn{1}{l|}{87.07}         & \multicolumn{1}{l|}{91.31}         & \multicolumn{1}{l|}{89.68}         & ($f_7$,$f_1$,$f_6$,$f_4$,$f_5$,$f_2$,$f_3$,$f_0$)                       & \multicolumn{1}{l|}{76.42}         & \multicolumn{1}{l|}{80.50}         & \multicolumn{1}{l|}{82.13}         & ($f_6$,$f_1$,$f_2$,$f_3$,$f_4$,$f_0$,$f_5$,$f_7$)                       \\ \hline
\textit{0,3,4}         & \multicolumn{1}{l|}{90.21}         & \multicolumn{1}{l|}{95.56}         & \multicolumn{1}{l|}{93.06}         & ($f_3$,$f_4$,$f_6$,$f_7$,$f_0$,$f_1$,$f_2$,$f_5$)                       & \multicolumn{1}{l|}{77.86}         & \multicolumn{1}{l|}{81.59}         & \multicolumn{1}{l|}{83.93}         & ($f_5$,$f_0$,$f_7$,$f_2$,$f_4$,$f_3$,$f_1$,$f_6$)                       \\ \hline
\textit{1,4,4}         & \multicolumn{1}{l|}{97.04}         & \multicolumn{1}{l|}{98.75}         & \multicolumn{1}{l|}{98.62}         & ($f_3$,$f_0$,$f_2$,$f_5$,$f_1$,$f_6$,$f_7$,$f_4$)                       & \multicolumn{1}{l|}{82.77}         & \multicolumn{1}{l|}{87.59}         & \multicolumn{1}{l|}{90.08}         & ($f_3$,$f_2$,$f_5$,$f_4$,$f_7$,$f_6$,$f_1$,$f_0$)                       \\ \hline
\textit{0,1,4}         & \multicolumn{1}{l|}{95.14}         & \multicolumn{1}{l|}{98.56}         & \multicolumn{1}{l|}{98.55}         & ($f_6$,$f_7$,$f_0$,$f_1$,$f_2$,$f_4$,$f_5$,$f_3$)                       & \multicolumn{1}{l|}{80.94}         & \multicolumn{1}{l|}{85.75}         & \multicolumn{1}{l|}{90.61}         & ($f_5$,$f_2$,$f_1$,$f_4$,$f_0$,$f_3$,$f_6$,$f_7$)                       \\ \hline
\textit{4,9,5}         & \multicolumn{1}{l|}{74.38}         & \multicolumn{1}{l|}{80.93}         & \multicolumn{1}{l|}{78.87}         & ($f_0$,$f_9$,$f_5$,$f_1$,$f_7$,$f_8$,$f_2$,$f_4$,$f_3$,$f_6$)           & \multicolumn{1}{l|}{65.42}         & \multicolumn{1}{l|}{68.68}         & \multicolumn{1}{l|}{70.35}         & ($f_2$,$f_6$,$f_9$,$f_4$,$f_1$,$f_5$,$f_8$,$f_3$,$f_0$,$f_7$)           \\ \hline
\textit{3,8,5}         & \multicolumn{1}{l|}{82.48}         & \multicolumn{1}{l|}{86.87}         & \multicolumn{1}{l|}{85.12}         & ($f_3$,$f_5$,$f_4$,$f_2$,$f_6$,$f_1$,$f_7$,$f_8$,$f_9$,$f_0$)           & \multicolumn{1}{l|}{69.98}         & \multicolumn{1}{l|}{73.6}          & \multicolumn{1}{l|}{76.03}         & ($f_0$,$f_6$,$f_7$,$f_9$,$f_2$,$f_8$,$f_4$,$f_1$,$f_5$,$f_3$)           \\ \hline
\textit{2,6,5}         & \multicolumn{1}{l|}{86.68}         & \multicolumn{1}{l|}{92.56}         & \multicolumn{1}{l|}{90.37}         & ($f_7$,$f_2$,$f_3$,$f_5$,$f_1$,$f_9$,$f_0$,$f_8$,$f_4$,$f_6$)           & \multicolumn{1}{l|}{73.31}         & \multicolumn{1}{l|}{76.73}         & \multicolumn{1}{l|}{79.65}         & ($f_8$,$f_7$,$f_0$,$f_2$,$f_1$,$f_6$,$f_5$,$f_9$,$f_3$,$f_4$)           \\ \hline
\textit{0,3,5}         & \multicolumn{1}{l|}{88.69}         & \multicolumn{1}{l|}{95.5}          & \multicolumn{1}{l|}{91.68}         & ($f_6$,$f_3$,$f_5$,$f_8$,$f_7$,$f_9$,$f_2$,$f_4$,$f_1$,$f_0$)           & \multicolumn{1}{l|}{73.38}         & \multicolumn{1}{l|}{78.08}         & \multicolumn{1}{l|}{81.73}         & ($f_3$,$f_5$,$f_0$,$f_9$,$f_1$,$f_6$,$f_2$,$f_7$,$f_8$,$f_4$)           \\ \hline
\textit{1,4,5}         & \multicolumn{1}{l|}{95.89}         & \multicolumn{1}{l|}{99.18}         & \multicolumn{1}{l|}{98.37}         & ($f_6$,$f_8$,$f_2$,$f_9$,$f_5$,$f_4$,$f_3$,$f_7$,$f_1$,$f_0$)           & \multicolumn{1}{l|}{79.31}         & \multicolumn{1}{l|}{83.81}         & \multicolumn{1}{l|}{86.25}         & ($f_3$,$f_8$,$f_2$,$f_1$,$f_6$,$f_9$,$f_0$,$f_7$,$f_5$,$f_4$)           \\ \hline
\textit{0,1,5}         & \multicolumn{1}{l|}{95.64}         & \multicolumn{1}{l|}{98.68}         & \multicolumn{1}{l|}{98.37}         & (($f_6$,$f_3$),($f_0$,$f_9$),($f_5$,$f_8$),($f_4$,$f_2$),($f_7$,$f_1$)) & \multicolumn{1}{l|}{78.75}         & \multicolumn{1}{l|}{86.33}         & \multicolumn{1}{l|}{87.0}          & (($f_4$,$f_1$),($f_9$,$f_5$),($f_0$,$f_2$),($f_7$,$f_3$),($f_8$,$f_6$)) \\ \hline
\end{tabular}
\end{table*}


We now present the results of the proposed GA. With $20$ population size and $5$ generations, the GA trains a total of $20 \times 5=100$ embedding permutations. For close comparison, we compare the performance of GA by randomly selecting $100$ embedding permutations and training them. This comparison is done for two datasets: MNIST and Tiny Imagenet \cite{le2015tiny} (reduced to lower dimension using UMAP \cite{leland2018uniform}). Additionally, we breakdown the analysis of results by low qubit count and high qubit count of the QNN. For low qubit count we select $3$, $4$ and $5$  qubits, while for high qubit count we choose $6$, $7$ and $8$ qubits for QNN. We present results for Tiny Imagenet to show scalability of the algorithm to larger dataset and high qubit count to show scalability in terms of number of qubits.

Overall, we do four different analyses: \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {\textbf{1}}}} \textit{low qubit count MNIST}, with binary classes $4-9$, $3-8$, $2-6$, $0-3$, $1-4$ and $0-1$, both noiseless and noisy conditions; \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {\textbf{2}}}} \textit{low qubit count Tiny Imagenet} with binary classes bell pepper-orange (SC$=$$0.05$) and sulphur butterfly-alp (SC$=$$0.51$) only noisy conditions; \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {\textbf{3}}}} \textit{high qubit count MNIST}, with binary classes $4-9$ and $0-1$, only noisy conditions; \raisebox{.5pt}{\textcircled{\raisebox{-.9pt} {\textbf{4}}}} \textit{high qubit count Tiny Imagenet} with binary classes bell pepper-orange and sulphur butterfly-alp, only noisy conditions. Compared to the other three analyses, the analysis performed in low qubit count MNIST case is the most extensive because it is has both less complex dataset as well as less number of qubits, which makes the analysis easier and more fundamental. As we shall see, the analyses for other cases can be extrapolated from this particular case with respect to the trend showed.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/0_1_4_results.pdf}
    \caption{Noiseless and Noisy plots for ($0$,$1$,$4$) MNIST case. Optmimal fitness score found by GA is highlighted on red line along with value.}
    \vspace{-5mm}
    \label{fig:0_1_4_results}
\end{figure}

\textbf{\textit{Low qubit count, MNIST:}} We tabulate the results for this scenario in Table \ref{tab:mnist_low_qubit_count}. Considering noiseless conditions we generally note that the best fitness score obtained from GA lies between the mean and best score of random selection, implying that GA finds a fitness score that is better than average random selection score and is generally close to the score of best performing randomly selected embedding permutation. For example for the case of binary classes $0$ and $1$ with $4$ qubit QNN ($0$,$1$,$4$), the GA finds an embedding permutation with fitness score ($98.55$) that is almost close to the score of best randomly chosen embedding permutation ($98.56$). However, when noise is taken into account random selection of embedding permutations yield poor fitness scores. The GA on the contrary, owing to its methodical evolutionary search of iteratively finding better embedding permutation in every successive generation succeeds in finding an optimum under noise that is better than the best performing randomly chosen embedding permutation. Considering once again the case ($0$,$1$,$4$), we see that the best randomly chosen embedding permutation has a fitness score of $85.75$ while GA selected embedding permutation has $90.61$. For illustrative purposes, we also show the histogram plots for randomly selected embedding permutations against the final GA fitness score for ($0$,$1$,$4$) case for both noiseless and noisy conditions in Fig. \ref{fig:0_1_4_results}. Additionally, we also note that this trend is consistent across all range of SC values of binary classes. Therefore, for remaining analyses, we restrict ourselves to two pairs of binary classes, one with low SC and other with high SC.

\textbf{\textit{Low qubit count, Tiny Imagenet:}}

\textbf{\textit{High qubit count, MNIST:}}

\textbf{\textit{High qubit count, Tiny Imagenet:}}

\subsection{Limitations}
% This point may not be needed! You can check and confirm.
A potential drawback of the proposed GA method is it's overall runtime. Assuming each embedding permutation takes average training time $T$, for population size  $s_{pop}$ and $g$ generations, the overall runtime would be $\mathcal{O}(s_{pop}.g.T)$. While $T$ is scalable to an extent (as we show by increasing the qubit count), the algorithm runtime would greatly increase if the search space of GA is expanded by increasing either $s_{pop}$ or $g$.  
% This point is definitely needed!
Additionally, the GA-based search outcome is valid for the chosen backend only (\textit{FakeBrisbane()} in this case). GA has to be rerun for a different specific backend e.g., \textit{FakeSherbrooke()}. A potential solution to this issue could be to gather data of best embedding permutation selected by GA for various coupling configurations across different hardware, and build a predictive model that takes input as the noise characteristics of the coupling configuration in the data gathered and would output the corresponding best embedding permutation. %This may sound counterintuitive at first because the potential solution would try to run GA for multiple hardware which is what we would want to avoid. However, once sufficient data is gathered, for rest of the desired coupling configurations that haven't been tested out the predictive model would then make predictions solely based on the noise data rather than rerunning the entire GA.

